Towards an Arrow-native Storage System

With the ever-increasing dataset sizes, several file formats like Parquet, ORC, and Avro have been developed to store data efficiently and to save network and interconnect bandwidth at the price of additional CPU utilization. However, with the advent of networks supporting 25-100 Gb/s and storage devices delivering 1, 000, 000 reqs/sec the CPU has become the bottleneck, trying to keep up feeding data in and out of these fast devices. The result is that data access libraries executed on single clients are often CPU-bound and cannot utilize the scale-out benefits of distributed storage systems. One attractive solution to this problem is to offload data-reducing processing and filtering tasks to the storage layer. However, modifying legacy storage systems to support compute offloading is often tedious and requires extensive understanding of the internals. Previous approaches re-implemented functionality of data processing frameworks and access library for a particular storage system, a duplication of effort that might have to be repeated for different storage systems. In this paper, we introduce a new design paradigm that allows extending programmable object storage systems to embed existing, widely used data processing frameworks and access libraries into the storage layer with minimal modifications. In this approach data processing frameworks and access libraries can evolve independently from storage systems while leveraging the scale-out and availability properties of distributed storage systems. We present one example implementation of our design paradigm using Ceph, Apache Arrow, and Parquet. We provide a brief performance evaluation of our implementation and discuss key results.

==> tex/7_acknowledgements.tex <==
\section{Acknowledgements}

This work was partially funded by the NSF Awards \#OAC-1836650 (IRIS-HEP), \#CNS-1764102, and \#CNS-1705021 as well as by the
Center for Research in Open Source Software (CROSS). We would like to thank everyone who has contributed code to this project.


==> tex/__extras__.tex <==

%%%%
\begin{comment}
In general, large-sized tabular datasets are often partitioned by certain columns to create a highly nested directory structure that allows partition pruning and helps optimize query execution \cite{costa2019evaluating}. Maintaining a directory structure requires filesystem metadata support which is not available in the RADOS layer in Ceph. Fortunately, Ceph provides a POSIX filesystem interface via CephFS that provides scalable metadata support and can be mounted as a local filesystem. Therefore, we decided to use CephFS as our file I/O layer where Parquet files are written in the local CephFS mount point. Although CephFS doesn't support directly accessing the objects in the RADOS layer which forms the backbone of our design, it provides access to rich metadata that contains information on how files in CephFS are mapped to objects in RADOS amongst many others. This information is termed as the striping strategy in Ceph. We leverage this striping strategy to translate filenames in the filesystem layer to object IDs in the RADOS layer and directly access these objects via Librados \cite{librados}, the client library for RADOS. In this way, besides having a filesystem view over the objects stored in RADOS, we also achieve the ability to interact with them directly in any way we like. Now that we have a high-level understanding of our design and the motivation behind it, we dive deep into the internals of the client and storage layer in the next section.
\end{comment}
%%%%


\begin{comment}
Ceph~\cite{weil2006ceph} is a popular example of a computational storage system~\cite{computationalstorage}. It is an open-source computational storage platform that implements object storage and provides a 3-in-1 interface for object, file, and block-level storage. Ceph provides an Object Class SDK that allows extending its RADOS (Object Store)~\cite{weil2007rados} interface with arbitrary functions for manipulating and accessing objects in ad-hoc ways. We leverage this feature of Ceph to create plugins in the form of shared libraries which we embed inside Ceph Object Storage Devices (OSDs).
This allows offloading CPU-bound operations, such as scanning to the storage layer. Although, the Object Class SDK makes it easy to implement functions for scanning Parquet files inside the storage nodes, implementing the actual file scanning logic requires format-specific access libraries and data processing abstractions. Apache Arrow~\cite{Arrow,ArrowDatasetDocs}, which is primarily an in-memory columnar format, also provides a set of APIs for common data processing tasks like applying query predicates and aggregation functions. Additionally, it provides APIs for reading tabular data from different file formats in an unified manner. We leverage these APIs provided by Arrow to build the data processing layer in our implementation. On the client side, we extend CephFS (the POSIX interface provided by Ceph)~\cite{borges2017cephfs} with APIs to directly access the objects that make up a file to be able to apply scan operations on a file within the storage layer.
\end{comment}
%probably, talk briefly about exposing our implementations via the Dataset API.

 
\begin{comment}
Examples of such storage systems are DAOS~\cite{liang2020daos}, OpenStack Swift~\cite{swift}, and Ceph. In our case, we use Ceph and extend both its client (Ceph Filesystem) and storage (Object Store) layers with externals plugins to enable offloading data processing. Our design also encourages the use of unified data processing frameworks like Apache Arrow, as they help integrate seamless (universal) data scanning functionality and allow users to easily extend the system to support different file formats.
\end{comment}
